A Domain-Specific Language and Editor for Parallel Particle Methods

Domain-specific languages (DSLs) are of increasing importance in scientific high-performance computing to reduce development costs, raise the level of abstraction and, thus, ease scientific programming. However, designing and implementing DSLs is not an easy task, as it requires knowledge of the application domain and experience in language engineering and compilers. Consequently, many DSLs follow a weak approach using macros or text generators, which lack many of the features that make a DSL a comfortable for programmers. Some of these features---e.g., syntax highlighting, type inference, error reporting, and code completion---are easily provided by language workbenches, which combine language engineering techniques and tools in a common ecosystem. In this paper, we present the Parallel Particle-Mesh Environment (PPME), a DSL and development environment for numerical simulations based on particle methods and hybrid particle-mesh methods. PPME uses the meta programming system (MPS), a projectional language workbench. PPME is the successor of the Parallel Particle-Mesh Language (PPML), a Fortran-based DSL that used conventional implementation strategies. We analyze and compare both languages and demonstrate how the programmer's experience can be improved using static analyses and projectional editing. Furthermore, we present an explicit domain model for particle abstractions and the first formal type system for particle methods.

==> Makefile <==
MAIN = paper_ppme_TOMS.tex
TEX = paper_ppme_TOMS.tex \
			preamble.tex \
			preface.tex \

SVGSRC = $(shell find $(CURDIR)/img -type f -name '*.svg')
SVGIMG = $(patsubst %.svg, %.pdf, $(SVGSRC))

paper: $(TEX) figures
	latexmk -pdf $(MAIN)

figures: ${SVGIMG}

%.pdf : %.svg
	inkscape --file=$*.svg --export-pdf=$*.pdf


clean:
	latexmk -c $(TEX)
	rm -f img/ppml-grayscott.pdf
	rm -f img/ppml-grayscott.aux
	rm -f img/ppml-grayscott.log
	rm -f img/ppme-populateRHS.pdf
	rm -f img/ppme-rhs_comparison.pdf
	rm -f ${SVGIMG}

distClean:
	latexmk -C $(TEX)



